Sigma term and strangeness content of octet baryons

By using lattice QCD computations we determine the sigma terms and strangeness content of all octet baryons by means of an application of the Hellmann-Feynman theorem. In addition to polynomial and rational expressions for the quark mass dependence of octet members, we use SU(3) covariant baryon chiral perturbation theory to perform the extrapolation to the physical up and down quark masses. Our N_f=2+1 lattice ensembles include pion masses down to about 190 MeV in large volumes (M_\pi L > 4), and three values of the lattice spacing. Our main results are the nucleon sigma term \sigma_{\pi N} = 39(4)(^{+18}_{-7}) and the strangeness content y_{N} = 0.20(7)(^{+13}_{-17}). Under the assumption of validity of covariant baryon \chi PT in our range of masses one finds y_{N} = 0.276(77)(^{+90}_{-62}).

==> chpt.tex <==

\newcommand{\pad}{\partial}
\newcommand{\til}{\tilde}
\newcommand{\pri}{^\prime}
\renewcommand{\dag}{^\dagger}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\trc}{\mathrm{tr}}
\newcommand{\Trc}{\mathrm{Tr}}
\newcommand{\Mpi}{M_\pi}
\newcommand{\Fpi}{F_\pi}
\newcommand{\Mka}{M_K}
\newcommand{\Fka}{F_K}
\newcommand{\Met}{M_\et}
\newcommand{\Fet}{F_\et}
\newcommand{\Mss}{M_{\bar{s}s}}
\newcommand{\Fss}{F_{\bar{s}s}}
\newcommand{\Mcc}{M_{\bar{c}c}}
\newcommand{\Fcc}{F_{\bar{c}c}}
\newcommand{\Mpibar}{\bar{M}_\pi}
\newcommand{\Mkabar}{\bar{M}_K}
\newcommand{\Metbar}{\bar{M}_\et}
\newcommand{\Mssbar}{\bar{M}_{\bar{s}s}}

\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand{\ep}{\epsilon}
\newcommand{\ve}{\varepsilon}
\newcommand{\ze}{\zeta}
\newcommand{\et}{\eta}
\renewcommand{\th}{\theta}
\newcommand{\vt}{\vartheta}
\newcommand{\io}{\iota}
\newcommand{\ka}{\kappa}
\newcommand{\la}{\lambda}
\newcommand{\rh}{\rho}
\newcommand{\vr}{\varrho}
\newcommand{\si}{\sigma}
\newcommand{\ta}{\tau}
\newcommand{\ph}{\phi}
\newcommand{\vp}{\varphi}
\newcommand{\ch}{\chi}
\newcommand{\ps}{\psi}
\newcommand{\om}{\omega}

\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\mr}{\mathrm}
\newcommand{\mb}{\mathbf}
\newcommand{\ri}{\mr{i}}
\newcommand{\MeV}{\,\mr{MeV}}
\newcommand{\GeV}{\,\mr{GeV}}
\newcommand{\fm}{\,\mr{fm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Sketch of the formalism of CBXPT}

To perform this calculation to ${\cal O}(p^3)$ we use the standard octet
baryon Lagrangians \cite{Jose}
\bea
{\cal L}_{MB}^{(1)}&=&\Trc\Big(
\ri{\overline B}\gamma^\mu D_\mu B-M_0{\overline B} B+
\frac{D}{2}{\overline B}\gamma^\mu\gamma_5\{u_\mu,B\}+
\frac{F}{2}{\overline B}\gamma^\mu\gamma_5[u_\mu,B]
\Big)
\label{p1}
\\
{\cal L}_{MB}^{(2)}&=&\Trc\Big(
b_D{\overline B}\{\chi_+,B\}+b_F{\overline B}[\chi_+,B]+\dots
\Big)+
b_0\Trc\Big({\overline B}B\Big)\Trc\Big(\chi_+\Big)+\ldots
\eea
with the chiral tensors
\bea
D_\mu B&=&\partial_\mu B+[\Gamma_\mu,B]
\\
\Gamma_\mu&=&\frac{1}{2}(u\dag(\pad_\mu+\ldots)u+u(\pad_\mu+\ldots)u\dag)
\\
u_\mu&=&\ri(u\dag(\pad_\mu+\ldots)u-u(\pad_\mu+\ldots)u\dag)
\\
\chi_\pm&=&u\dag\chi u\dag\pm u\chi\dag u
\\
\chi&=&2B_0(M+\ldots)
\eea
where $M$ denotes the (diagonal) quark mass matrix.
To the order we are working, there is no contribution from
${\cal L}_{MB}^{(3)}$ to the quark-mass dependence of the octet baryon masses.
In Eq.\,(\ref{p1}) the coupling constants $D,F$ denote SU(3) axial-couplings of
a baryon in the chiral limit, whereas $M_0$ corresponds to the chiral limit
value of the mass of the baryon octet.
The field $u(x)=\sqrt{U(x)}$ describes a non-linear matrix representation of
the (quasi-) Goldstone boson fields and $B$ is the matrix-valued interpolating
field for a spin 1/2 octet baryon.
The next-to-leading order low-energy constants $b_D,b_F,b_0$ govern the leading
quark-mass contributions to the mass of a spin 1/2 octet baryon, with
${\cal M}$ denoting the quark-mass matrix for three light flavors $u,d,s$.
Furthermore, we note that the parameter $B_0$ is a measure of the size of the
chiral condensate $\<0|\bar{q}q|0\>$ (in the chiral limit) \cite{GL84}
\beq
B_0\equiv-\,\frac{\<0|\bar{q}q|0\>_{m_q\to0}}{F_0^2}
\eeq
where the low energy constant $F_0$ is identified with the value of the octet
Goldstone Boson decay constant in the chiral limit.
Finally, for the calculation at hand one needs to know the chiral meson
Lagrangian up to ${\cal O}(p^2)$ \cite{GL84}
\bea
{\cal L}_{M}^{(2)}&=&\frac{F_0^2}{4}
\Trc\{(\pad_\mu+\ldots) U\dag(\pad^\mu+\ldots) U+\chi\dag U+\chi U\dag\}
\eea
After this brief summary of the relevant XPT formalism we move on to a
discussion of chiral extrapolation functions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Chiral expansion for the nucleon mass}

The leading one-loop result for the calculation of the mass of a nucleon to
${\cal O}(p^3)$ in Baryon ChPT reads \cite{}
\bea
M_N&=&M_0-4(b_0+(b_D+b_F)/2)\Mpibar^2-2(b_0+b_D-b_F)\Mssbar^2
\nonumber\\
&-&\frac{\til{g}_{\pi N}\,\Mpibar^3}{4\pi^2F_A^2}
\Big\{\sqrt{1-\frac{\Mpibar^2}{4M_0^2}}\arccos{\frac{\Mpibar}{2M_0}}+
\frac{\Mpibar}{4M_0}\log\frac{\Mpibar^2}{M_0^2}\Big\}
\nonumber\\
&-&\frac{\til{g}_{K N}\,\Mkabar^3}{4\pi^2F_B^2}
\Big\{\sqrt{1-\frac{\Mkabar^2}{4M_0^2}}\arccos{\frac{\Mkabar}{2M_0}}+\
\frac{\Mkabar}{4M_0}\log\frac{\Mkabar^2}{M_0^2}\Big\}
\nonumber\\
&-&\frac{\til{g}_{\et N}\,\Metbar^3}{4\pi^2F_C^2}\Big\{
\sqrt{1-\frac{\Metbar^2}{4M_0^2}}\arccos{\frac{\Metbar}{2M_0}}+
\frac{\Metbar}{4M_0}\log\frac{\Metbar^2}{M_0^2}\Big\}+{\cal O}(p^4)
\label{m3}
\eea
To the chiral order we are working here, the three couplings
$\til{g}_{\pi N},\til{g}_{KN},\til{g}_{\et N}$ can be expressed in terms of the
two SU(3) parameters $F$ and $D$, as given in Tab.\,\ref{tab:gmb}.
The ${\cal O}(p^3)$ result of Eq.(\ref{m3}) was obtained by generalizing the
corresponding SU(2) Baryon ChPT result of ref.\cite{DGH,IRbar} to the case of
3 flavors, utilizing the same (modified) infrared regularization approach.
Finally, we note that we have expressed the Goldstone boson decay constant
$F_0$ entering the loop contributions via three different symbols
$F_A,F_B,F_C$ to better account for the individual contribution of the pion,
kaon and eta-cloud of the nucleon, as discussed below.

\begin{table}[tb]
\centering
\begin{tabular}{|c|cccc|}
\hline
$g_{M\!B}$ & $N$ & $\Lambda$ & $\Sigma$ & $\Xi$ \\
\hline
$\pi$ & $\frac{3}{4}(D\!+\!F)^2$ & $D^2$ &
        $\frac{1}{3}(D^2\!+\!6F^2)$ & $\frac{3}{4}(D\!-\!F)^2$\\
$K$   & $\frac{1}{6}(5D^2\!-\!6DF\!+\!9F^2)$ & $\frac{1}{3}(D^2\!+\!9F^2)$ &
        $(D^2\!+\!F^2)$ & $\frac{1}{6}(5D^2\!+\!6DF\!+\!9F^2)$ \\
$\et$ & $\frac{1}{12}(D\!-\!3F)^2$ & $\frac{1}{3}D^2$ &
        $\frac{1}{3}D^2$ & $\frac{1}{12}(D\!+\!3F)^2$\\
\hline
\end{tabular}
\caption{\small\sl Summary of meson-baryon couplings $g_{MB}$ in terms of the
low-energy constants $D,F$.}
\label{tab:gmb}
\end{table}

For a fit to lattice QCD data we advocate the following changes (which, of
course, are consistent with the perturbative chiral expansion to the order at
which we work here):
\begin{enumerate}
\item
We express the GOR-masses for $\Mkabar,\Metbar$ in Eq.(\ref{m3}) as a function
of the GOR-mass of the pion and of the mass-parameter $\Mssbar$ introduced in
Eq.\,(\ref{Mss}):
\begin{eqnarray}
\Mkabar^2&\to&\frac{1}{2}(\Mpibar^2+\Mssbar^2)
\\
\Metbar^2&\to&\frac{1}{3}(\Mpibar^2+2\Mssbar^2)
\end{eqnarray}
This just amounts to a change of variables without introducing any approximations.
\item
In a second step we identify the GOR-mass $\Mpibar$ of Eq.\,(\ref{Mss}) with
the corresponding lowest-lying $0^-$-boson mass $\Mpi$ observed on the lattice.
Possible deviations in the quark-mass dependence from the linear GOR-behavior
predicted in Eq.(\ref{Mss}) can only affect ${\cal O}(p^4)$ (and higher
order) corrections to Eq.\,(\ref{m3}).
\item
The Goldstone Boson decay constants $F_A,F_B,F_C$ in Eq.\,(\ref{m3}) can either
be identified with the common SU(3) decay constant $F_0$ in the 3-flavor chiral
limit or with the value of \emph{one} of the decay constants at the physical
point (e.g.\ $\Fka^\mr{phys}$) or with the corresponding ``local'' values given
at the respective quark-masses.
Once more, we emphasize that the difference between these 3 possible
assignments is of higher order.
When fitting the chiral extrapolation function to the lattice data in we will
study the differences between the latter two assignments.
The relevant quark-mass dependencies of $F_A\to\Fpi,F_B\to\Fka,F_C\to\Fet$ are
given in App.\,\ref{GBdecay}.
\item
With the same reasoning as in the previous item, at chiral order
${\cal O}(p^3)$ we can identify the chiral limit couplings
$\til{g}_{\pi N},\til{g}_{KN},\til{g}_{\et N}$ with the physical couplings
$g_{\pi N},g_{KN},g_{\et N}$, resulting in Tab.\,\ref{tab:gxa}.
The unknown ratio $\xi$ of the physical $F^\mr{phys}/D^{phys}$ couplings is
treated as an external input to our fits.
We use $\xi=2/3$ \cite{FoD} and study the influence of possible deviations from
this value%
\footnote{Note that SU(3) symmetry breaking corrections to a universal $F/D$
ratio discussed in the literature \cite{symbreaking} only affect higher order
chiral corrections to our BChPT result; in fact they start at ${\cal O}(p^5)$.}.
We note that unlike in the case of the Goldstone boson decay constants we do
not study the influence of a quark-mass dependence of these 3 couplings, as we
do not possess the corresponding lattice data.
Therefore we fix these couplings at their values at the physical point for all
our fits.
In support of this choice, we note that extensive lattice studies \cite{gA}
of the observable $g_A\equiv\sqrt{4g_{\pi N}/3}$ have shown that the
quark-mass dependence of this coupling is flat, albeit with a large
normalization uncertainty.
Furthermore, recent studies \cite{Lin} of the quark-mass dependence of the
hyperon couplings also suggest that their dependence on the light quark-mass is
rather weak, in favor of the approach chosen here.
\end{enumerate}
With these four changes, the chiral extrapolation formula at leading-one-loop
order for the mass of a nucleon reads
\bea
M_N&=&M_0-4(b_0+(b_D+b_F)/2)\Mpi^2-2(b_0+b_D-b_F)\Mss^2
\nonumber\\
&+&\frac{g_{\pi N}}{\Fpi^2}H[\Mpi^2]
  +\frac{g_{KN}}{\Fka^2}H[\frac{\Mpi^2\!+\!\Mss^2}{2}]
  +\frac{g_{\et N}}{\Fet^2}H[\frac{\Mpi^2\!+\!2\Mss^2}{3}]
  +4\de_\pi \Mpi^4+4\de_s \Mss^4
\label{mN}
\eea
Here the two terms governed by $\de_\pi,\de_s$ have been introduced to
parameterize the possible corrections of chiral order ${\cal O}(p^4)$, while
the quantum-loop effects due to the Goldstone bosons of mass $m$ are given by
the function
\beq
H[m^2]=-\,\frac{m^3}{4\pi^2}
\Big\{\sqrt{1-\frac{m^2}{4M_0^2}}\arccos{\frac{m}{2M_0}}+
\frac{m}{4M_0}\log\frac{m^2}{M_0^2}\Big\}
\eeq
\emph{but personally I would prefer to write}
\bea
M_N\!&\!=\!&\!M_0-4(b_0\!+\!(b_D\!+\!b_F)/2)\Mpi^2-2(b_0\!+\!b_D\!-\!b_F)\Mss^2
\nonumber
\\
\!&\!-\!&\!4M_0\frac{g_{\pi N}\Mpi^2}{(4\pi\Fpi)^2}h(x_\pi)
  -4M_0\frac{g_{KN}\Mka^2}{(4\pi\Fka)^2}h(x_K)
  -4M_0\frac{g_{\et N}\Met^2}{(4\pi\Fet)^2}h(x_\et)
  +4\de_\pi \Mpi^4+4\de_s \Mss^4
\eea
with
\beq
h(x)=x\Big\{\sqrt{1-\frac{x^2}{4}}\arccos\Big(\frac{x}{2}\Big)
+\frac{x}{4}\log\Big(x^2\Big)\Big\}
\eeq
and $x_M\!\equiv\!M_M/M_0$ for $M=\pi,K,\et$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Chiral expansion for the masses of the octet hyperons}

Performing the same analysis steps as outlined in the previous subsection, the
result for the quark-mass dependence of the mass of a $\Lambda$, $\Sigma$ and
$\Xi$hyperon to ${\cal O}(p^3)$ in CBXPT reads
\bea
M_\Lambda&=&M_0-4(b_0+\frac{b_D}{3})\Mpi-2(b_0+\frac{4b_D}{3})\Mss^2
\nonumber\\
&+&\frac{g_{\pi\Lambda}}{\Fpi^2}H[\Mpi^2]
+\frac{g_{K\Lambda}}{\Fka^2}H[\frac{\Mpi^2\!+\!\Mss^2}{2}]
+\frac{g_{\et\Lambda}}{\Fet^2}H[\frac{\Mpi^2\!+\!2\Mss^2}{3}]
+4\de_\pi\Mpi^4+4\de_s\Mss^4
\label{mLambda}
\\
M_\Sigma&=&M_0-4(b_0+b_D)\Mpi^2-2b_0\Mss^2
\nonumber\\
&+&\frac{g_{\pi\Sigma}}{\Fpi^2}H[\Mpi^2]
+\frac{g_{K\Sigma}}{\Fka^2}H[\frac{\Mpi^2\!+\!\Mss^2}{2}]
+\frac{g_{\et\Sigma}}{\Fet^2}H[\frac{\Mpi^2\!+\!2\Mss^2}{3}]
+4\de_\pi\Mpi^4+4\de_s\Mss^4
\label{mSigma}
\\
M_\Xi&=&M_0-4(b_0+\frac{b_D}{2}-\frac{b_F}{2})\Mpi^2-2(b_0+b_D+b_F)\Mss^2
\nonumber\\
&+&\frac{g_{\pi\Xi}}{\Fpi^2}H[\Mpi^2]
+\frac{g_{K\Xi}}{\Fka^2}H[\frac{\Mpi^2\!+\!\Mss^2}{2}]
+\frac{g_{\et\Xi}}{\Fet^2}H[\frac{\Mpi^2\!+\!2\Mss^2}{3}]
+4\de_\pi\Mpi^4+4\de_s\Mss^4
\label{mXi}
\eea
Obviously the general structure is identical to the analogous expression for
the mass of a nucleon in Eq.(\ref{mN}).
Aside from the (unknown) chiral-limit SU(3) multiplet mass $M_0$ the leading
quark-mass dependence is governed by the three LECs $b_0,b_D,b_F$.
The relevant $g$-couplings can be found in Table \ref{tab:gxa}, while the
quark-mass dependence of the Goldstone boson decay constants $\Fpi,\Fka,\Fet$
is discussed in Appendix \ref{GBdecay}.
Once more we have also added the leading corrections of ${\cal O}(p^4)$ via the
two $\de-$parameters.

\bea
M_N&=&M_0-2(2b_0+b_D+b_F)\Mpi^2-2(b_0+b_D-b_F)\Mss^2
\nonumber
\\
&&
+\frac{g_{\pi N}}{\Fpi^2}H(\Mpi^2)
+\frac{g_{K   N}}{\Fka^2}H(\Mka^2)
+\frac{g_{\et N}}{\Fet^2}H(\Met^2)
+4\de_\pi\Mpi^4+4\de_{\bar{s}s}\Mss^4
\label{hemmert1}
\\
M_\Lambda&=&M_0-4(b_0+b_D/3)\Mpi^2-2(b_0+4b_D/3)\Mss^2
\nonumber
\\
&&
+\frac{g_{\pi \Lambda}}{\Fpi^2}H(\Mpi^2)
+\frac{g_{K   \Lambda}}{\Fka^2}H(\Mka^2)
+\frac{g_{\et \Lambda}}{\Fet^2}H(\Met^2)
+4\de_\pi\Mpi^4+4\de_{\bar{s}s}\Mss^4
\label{hemmert2}
\\
M_\Sigma&=&M_0-4(b_0+b_D)\Mpi^2-2b_0\Mss^2
\nonumber
\\
&&
+\frac{g_{\pi \Sigma}}{\Fpi^2}H(\Mpi^2)
+\frac{g_{K   \Sigma}}{\Fka^2}H(\Mka^2)
+\frac{g_{\et \Sigma}}{\Fet^2}H(\Met^2)
+4\de_\pi\Mpi^4+4\de_{\bar{s}s}\Mss^4
\label{hemmert3}
\\
M_\Xi&=&M_0-2(2b_0+b_D-b_F)\Mpi^2-2(b_0+b_D+b_F)\Mss^2
\nonumber
\\
&&
+\frac{g_{\pi \Xi}}{\Fpi^2}H(\Mpi^2)
+\frac{g_{K   \Xi}}{\Fka^2}H(\Mka^2)
+\frac{g_{\et \Xi}}{\Fet^2}H(\Met^2)
+4\de_\pi\Mpi^4+4\de_{\bar{s}s}\Mss^4
\label{hemmert4}
\eea

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Finite volume corrections for masses of the octet hyperons}

In general, the mass $M_B(\Mpi^2,\Mss^2,L)$ of an octet baryon
$B=N,\Lambda,\Sigma,\Xi$ obtained in lattice QCD simulations with 2+1 light
quark flavors exceeds the mass $M_B(\Mpi^2,\Mss^2)$ in infinite volume by
an excess
\begin{equation}
\Delta M_B(\Mpi^2,\Mss^2,L)=M_B(\Mpi^2,\Mss^2,L)-M_B(\Mpi^2,\Mss^2)
\end{equation}
When determining $\Delta M_B(\Mpi^2,\Mss^2,L)$ in this work we follow the
{\it direct approach} of \cite{QCDSF04}, i.e.\ we evaluate the finite volume
effects from the relevant Feynman diagrams of ${\cal O}(p^3)$ in a finite
volume with periodic boundary conditions within BXPT%
\footnote{Alternatively, one could evaluate $\Delta M_B(\Mpi^2,\Mss^2,L)$ via
the SU(3) meson-baryon scattering amplitudes as proposed in \cite{Luscher:1985dn}.}.
We obtain
\begin{eqnarray}
\Delta M_N(\Mpi^2,\Mss^2,L)\!&\!=\!&\!
\frac{g_{\pi N}}{\Fpi^2}\,G[\Mpi^2]
+\frac{g_{KN}}{\Fka^2}\,G[\frac{\Mpi^2\!+\!\Mss^2}{2}]
+\frac{g_{\et N}}{\Fet^2}\,G[\frac{\Mpi^2\!+\!2\Mss^2}{3}]
+{\cal O}(p^4)\qquad\label{a}
\\
\Delta M_\Lambda(\Mpi^2,\Mss^2,L)\!&\!=\!&\!
\frac{g_{\pi\Lambda}}{\Fpi^2}\,G[\Mpi^2]
+\frac{g_{K\Lambda}}{\Fka^2}\,G[\frac{\Mpi^2\!+\!\Mss^2}{2}]
+\frac{g_{\et\Lambda}}{\Fet^2}\,G[\frac{\Mpi^2\!+\!2\Mss^2}{3}]
+{\cal O}(p^4)\qquad\label{b}
\\
\Delta M_\Sigma(\Mpi^2,\Mss^2,L)\!&\!=\!&\!
\frac{g_{\pi\Sigma}}{\Fpi^2}\,G[\Mpi^2]
+\frac{g_{K\Sigma}}{\Fka^2}\,G[\frac{\Mpi^2\!+\!\Mss^2}{2}]
+\frac{g_{\et\Sigma}}{\Fet^2}\,G[\frac{\Mpi^2\!+\!2\Mss^2}{3}]
+{\cal O}(p^4)\qquad\label{c}
\\
\Delta M_\Xi(\Mpi^2,\Mss^2,L)\!&\!=\!&\!
\frac{g_{\pi\Xi}}{\Fpi^2}\,G[\Mpi^2]
+\frac{g_{K\Xi}}{\Fka^2}\,G[\frac{\Mpi^2\!+\!\Mss^2}{2}]
+\frac{g_{\eta\Xi}}{\Fet^2}\,G[\frac{\Mpi^2\!+\!2\Mss^2}{3}]
+{\cal O}(p^4)\qquad\label{d}
\end{eqnarray}
with the coupling constants given in Table \ref{tab:gxa} and the quark-mass
dependence of the Goldstone boson decay constants discussed in appendix
\ref{GBdecay}.
Note that the finite volume correction via the {\it direct method} only starts
at ${\cal O}(p^3)$ in the effective field theory calculation and therefore only
amounts to the leading contributions in each channel%
\footnote{The next-to-leading order finite volume corrections to the baryon
masses are also known, albeit only for the case of 2 flavor QCD \cite{IRbar}.
Given the relatively large values of $m_\pi L$ in the BMW-data, we expect
Eqs.(\ref{a}-\ref{d}) to be well-sufficient for the required finite volume
corrections.}
In the modified infrared regularization scheme employed here the result for
function $G[m^2]$ is identical to the result one would obtain in the
usual $\overline{\mr{MS}}$ approach, where $m$ refers to the mass of the meson
affected by the boundary conditions and $M_0$ denotes the mass of the baryon in
the chiral limit:
\beq
G[m^2]=\frac{M_0}{4\pi^2}\int_0^1\!dt\,
\sum\nolimits_{\vec{n}}^\prime
\Big\{
m^2\,K_0\Big(|\vec{n}|\sqrt{M_0^2t^2\!+\!m^2(1\!-\!t)}\,L\Big)-
2M_0^2\,\frac{K_1(|\vec{n}|M_0L)}{|\vec{n}|M_0L}
\Big\}
\eeq
The functions $K_i$ denote the usual Bessel-functions of finite volume ChPT.
Note that the ``zero-mode'' $(0,0,0)$ is omitted from the threefold sum over
the discrete momentum label $\vec{n}\in\mb{Z}^3$.

\begin{thebibliography}{99}
\bibitem{GL84} J. Gasser and H. Leutwyler, Nucl. Phys. {\bf B250}, 465 (1984).
\bibitem{Jose} {\it e.g.} see J.A. Oller, J. Prades and M. Verbeni, JHEP 0609, 079 (2006); M. Frink and U.-G. Mei{\ss}ner, Eur. Phys. J. {\bf A29}, 255 (2006); J.A. Oller, J. Prades and M. Verbeni, JHEP-Erratum 0609, 079 (2006).
%\bibitem{Bugra} B. Borasoy U.-G. Mei{\ss}ner, Ann. Phys. {\bf 254}, 192 (1997).
%\bibitem{Frink2} M. Frink, U.-G. Mei{\ss}ner and I. Scheller, Eur. Phys. J. {\bf A24}, 395 (2005).
%\bibitem{PHW04} M. Procura, T.R. Hemmert and W. Weise, Phys. Rev. {\bf D69}, 034505 (2004).
\bibitem{QCDSF04} QCDSF-UKQCD Collaboration (A. Ali Khan et al.), Nucl. Phys. {\bf B689}, 175 (2004).
%\bibitem{Frink} M. Frink and U.-G. Mei{\ss}ner, JHEP 0407, 028 (2004).
%\bibitem{PDG} C. Amsler et al. (Particle Data Group), Phys. Lett. {\bf B667}, 1 (2008).
\bibitem{DGH} M. Dorati, T.A. Gail and T.R. Hemmert, Nucl. Phys. {\bf A798}, 96 (2008).
\bibitem{IRbar} T.A. Gail and TRH, in preparation.
\bibitem{gA} recent gA studies: QCDSF proceedings, LHPC, RBC
\bibitem{FoD} source of F/D=2/3
\bibitem{symbreaking} F/D symmetrie-breaking effects from Andreas and lattice study by Lin et al.
\bibitem{Lin} {\it e.g.} see H.-W. Lin, Nucl. Phys. Proc. Suppl.{\bf 187}, 200 (2009) and references given therein.
%\bibitem{fGBstudies} recent studies of fpi, fK
%\bibitem{Tony} reference to log-modification of the Adelaide group
%\bibitem{sigmastudies} previous studies of piN-sigma term from lattice QCD
%\bibitem{fTsstudies} previous studies of fTs from lattice QCD
%\bibitem{KNsigma} studies of KN sigma term from Kaonic atoms
\end{thebibliography}

\section{Decay constants of Goldstone bososns\label{GBdecay}}

\emph{I think there is no point in summarizing these standard formulas.}

